Defending Pre-trained Language Models as Few-shot Learners against Backdoor Attacks

Pre-trained language models (PLMs) have demonstrated remarkable performance as few-shot learners. However, their security risks under such settings are largely unexplored. In this work, we conduct a pilot study showing that PLMs as few-shot learners are highly vulnerable to backdoor attacks while existing defenses are inadequate due to the unique challenges of few-shot scenarios. To address such challenges, we advocate MDP, a novel lightweight, pluggable, and effective defense for PLMs as few-shot learners. Specifically, MDP leverages the gap between the masking-sensitivity of poisoned and clean samples: with reference to the limited few-shot data as distributional anchors, it compares the representations of given samples under varying masking and identifies poisoned samples as ones with significant variations. We show analytically that MDP creates an interesting dilemma for the attacker to choose between attack effectiveness and detection evasiveness. The empirical evaluation using benchmark datasets and representative attacks validates the efficacy of MDP.

==> analysis.tex <==
\section{Extra Analysis}
% In this section, we first analyze the impact of different hyper-parameter settings, and then
% conduct the ablation study. Finally, we explore the performance of the proposed method under adaptive attacks.

% \subsection{Sensitivity Analysis}

% \textbf{Effects of the Mask Ratio.}
% We also study the effects of the mask ratio on \system's performance. Figure x shows the performance of \system with different mask ratio. It can be seen that xxx
% As we can observe, 

% \textbf{Effects of Trigger Length.} 
% In this experiment, we study the influence of trigger length (i.e., the number of tokens in each trigger) on the defense performance. To this end, we conduct experiments on x dataset. Since longer triggers are more likely to be visible, we only vary the length of each trigger from x to x. Figure x shows the defense performance with different trigger lengths. It can be seen that there is a trend of xxx when we increase the trigger length.

% \subsection{Ablation Study}
% In the ablation study, we investigate the effect of \system without the proposed prompt optimization or xxx. We conduct ablation studies on the xxx dataset. The hyper-parameters (i.e., the trigger length and mask ratio) are set according to xxx.

% Table x shows the results of the ablation study. The best performance is highlighted in bold. Overall, it can be seen that \system with prompt optimization has a better performance than \system without prompt optimization in terms of evaluation metrics. It validates the motivation that by xxx ...

\subsection{Theoretical Analysis}
The empirical evaluation above shows \system's superior performance in defending textual backdoor attacks under the few-shot learning scenario. Next, we provide a theoretical analysis of its effectiveness. Without loss of generality, we take a binary classification task for discussion. 

Assume the label to protect is $y_T$, which can be either 0 or 1. The backdoored model classifies $X_\mathrm{in}$ as the target label $y_T$ if $p_\theta(y_T | X_\mathrm{in}) > \frac{1}{2}$. 
Suppose there is a poisoned input $X_\mathrm{in}$ that has $N$ random masked versions $\sboth{\hat{X}}{\mathrm{in}}{\mathrm{1}}, \sboth{\hat{X}}{\mathrm{in}}{\mathrm{2}}, \cdots, \sboth{\hat{X}}{\mathrm{in}}{\mathrm{N}}$, among which there is only one version $\sboth{\hat{X}}{\mathrm{in}}{\mathrm{k}}$ whose trigger has been masked, thus it would not be predict as 
$y_T$, i.e., $p_\theta(y_T | \sboth{\hat{X}}{\mathrm{in}}{\mathrm{k}}) \leq \sigma_2 < \frac{1}{2}$. Meanwhile, the remain $N-1$ masked versions of which the trigger words are not masked would still be classified as $y_T$, i.e., $p_\theta(y_T | \sboth{\hat{X}}{\mathrm{in}}{\mathrm{i}}) \geq \sigma_1 > \frac{1}{2}, i \neq k$.


Assume $p_\theta$ satisfies the following conditions:
(1) $p_\theta(y_T | X_\mathrm{in}) \geq \sigma_1 > \frac{1}{2}$;
(2) $\forall $




% Denote a clean given input $X$, a poisoned input $X'$ , mask $M$, 
% % $$p(y_T | X_\mathrm{clean}) - p(y_T | X_\mathrm{clean} \odot M)$$
% difference $$\Delta_{p,p'} \triangleq (p([{\tt mask}] |  X \odot M),p([{\tt mask}] |  X' \odot M)) $$
% where $\odot$ denotes element-wise multiplication, $\Delta$ can be any distribution distance metric such as KL-divergence.

% \begin{theorem}
% Define $\gD$, 
% \end{theorem}

% The masking-invariant prompt training objective:
% \begin{equation}
%     \operatorname*{arg\,min}_\theta [\gL( f(X; \theta),y) + \gL( f(X \odot M; \theta),y_T)]
% \end{equation}

% For the attacker that wants to evade \system, their attack objective can be formulated as minimizing the following optimization problem:
% \begin{equation}
%     \gL(f(X;\theta),y) + \gL(f(X';\theta),y_T) + \Delta_{p,p'}
% \end{equation}

% \textbf{Trade-off between Attack Performance and Detection Evasiveness.}
% We theoretically analyze the trade-off caused by \system between attack performance and detection evasiveness. 







% From eq.x, we can see that $\alpha=0$ is equivalent to the original model, and $\alpha=1$ means that we exclusively use the masked inputs and completely do not consider the original task. $\alpha$ presents a original-defense performance trade-off: $\alpha \downarrow 0$ means higher original performance, $\alpha \uparrow 1$ means better backdoor defense performance.

% \subsection{Adaptive Attacks}
% We study the scenario where the adversary has knowledge of the mechanism of \system and aims to bypass it. In the adaptive attack, the attacker ... Table x shows the defense performance under the adaptive attack.


